Mention Memory: incorporating textual knowledge into Transformers through entity mention attention

Natural language understanding tasks such as open-domain question answering often require retrieving and assimilating factual information from multiple sources. We propose to address this problem by integrating a semi-parametric representation of a large text corpus into a Transformer model as a source of factual knowledge. Specifically, our method represents knowledge with `mention memory', a table of dense vector representations of every entity mention in a corpus. The proposed model - TOME - is a Transformer that accesses the information through internal memory layers in which each entity mention in the input passage attends to the mention memory. This approach enables synthesis of and reasoning over many disparate sources of information within a single Transformer model. In experiments using a memory of 150 million Wikipedia mentions, TOME achieves strong performance on several open-domain knowledge-intensive tasks, including the claim verification benchmarks HoVer and FEVER and several entity-based QA benchmarks. We also show that the model learns to attend to informative mentions without any direct supervision. Finally we demonstrate that the model can generalize to new unseen entities by updating the memory without retraining.

==> results/tqa_samples.tex <==
\begin{table}[t!]
\centering
\caption{Top retrieval samples for TriviaQA questions. \label{table:mention_retrieval_samples}}
\begin{tabularx}{\textwidth}{Xr}
\toprule
Questions & Answer \\
\midrule
Who had an 80s no 1 hit with Hold on to the nights? & Marx,\_Richard \\
$\longrightarrow$ \ldots the song reached number 2 on the us billboard hot 100 (denied the top spot by "hold on to the nights" by  \textbf{[richard marx]}), \ldots \\
\midrule
Who had an 80s no 1 hit with Hold on to the nights? & Marx,\_Richard \\
$\longrightarrow$ \ldots the song reached number 2 on the us billboard hot 100 (denied the top spot by "hold on to the nights" by  \textbf{[richard marx]}), \ldots \\
\midrule
Who had an 80s no 1 hit with Hold on to the nights? & Marx,\_Richard \\
$\longrightarrow$ \ldots the song reached number 2 on the us billboard hot 100 (denied the top spot by "hold on to the nights" by  \textbf{[richard marx]}), \ldots \\
\bottomrule
\end{tabularx}
\end{table}

==> results/tqa_subset.tex <==
\begin{tabular}{l|cccc}
\toprule
Model & Recall@20 \\
\midrule
Entities as Experts & 61.1 \\
DPR & 65.4 \\
BM25 & 71.2 \\
\tome-1 & 83.3 \\
\tome-2 & 83.8\\
\bottomrule
\end{tabular}

==> results/unnamed_example.tex <==
\begin{tabularx}{\textwidth}{X}
\toprule
Claim: \textbf{The song} recorded by  \textbf{Fergie} that was produced by  \textbf{Polow Da Don} and was followed by  \textbf{Life Goes On} was \textbf{M.I.L.F.}. Label: TRUE \\ 
\midrule
Superdrag $\longrightarrow$ Superdrag was an American alternative rock band from Knoxville, Tennessee, United States. \dots. Early years (1992-1995) \textbf{[Superdrag]} formed in the early 1990s when knoxville guitar player brandon fisher began dating the cousin of john davis. \ldots \\
Collective Soul $\longrightarrow$ \ldots Collective Soul is an American rock band originally from Stockbridge, Georgia. \ldots. Before forming  \textbf{[Collective Soul]}, singer Ed Roland studied music composition and guitar at the Berklee college of music in Boston, Massachusetts. \\
rock band $\longrightarrow$ \ldots A group of musicians performing rock music is termed as a \textbf{[rock band]} or a rock group. Furthermore, it typically consists of between three (the power trio) and five members.\\
\bottomrule
\end{tabularx}
